Characterizing Exoplanet Atmospheres: From Light-curve Observations to Radiative-transfer Modeling

Multi-wavelength transit and secondary-eclipse light-curve observations are some of the most powerful techniques to probe the thermo-chemical properties of exoplanets. Although the large planet-to-star brightness contrast and few available spectral bands produce data with low signal-to-noise ratios, a Bayesian approach can robustly reveal what constraints we can set, without over-interpreting the data. Here I performed an end-to-end analysis of transiting exoplanet data. I analyzed space-telescope data for three planets to characterize their atmospheres and refine their orbits, investigated correlated noise estimators, and contributed to the development of the respective data-analysis pipelines. Chapters 2 and 3 describe the Photometry for Orbits, Eclipses and Transits (POET) pipeline to model Spitzer Space Telescope light curves, applied to secondary-eclipse observations of the Jupiter-sized planets WASP-8b and TrES-1. Chapter 4 studies commonly used correlated-noise estimators for exoplanet light-curve modeling, time averaging, residual permutations, and wavelet likelihood, and assesses their applicability and limitations to estimate parameters uncertainties. Chapter 5 describes the open-source Bayesian Atmospheric Radiative Transfer (BART) code to characterize exoplanet atmospheres. BART combines a thermochemical-equilibrium code, a one-dimensional line-by-line radiative-transfer code, and the Multi-core Markov-chain Monte Carlo statistical module to constrains the atmospheric temperature and chemical-abundance profiles of exoplanets. I applied the BART code to the Hubble and Spitzer Space Telescope transit observations of the Neptune-sized planet HAT-P-11b. BART finds an atmosphere enhanced in heavy elements, constraining the water abundance to ~100 times that of the solar abundance.

==> latbibucf <==
#! /bin/bash

root=$1

#if [ -d /usr/share/texmf-texlive ]; then
#  tex_dir=/usr/share/texmf-texlive
#else
#  tex_dir=/usr/share/texmf-tetex
#fi

#export TEXFONTS=.:/home/jh/lib/texmf/fonts//:${tex_dir}/fonts//
#export TEXINPUTS=.:/home/jh/lib/texmf/tex//:${tex_dir}/tex//
#export BIBINPUTS=.:/home/jh/ast/papers/bib//:/home/jh/lib/texmf/bibtex/bib//:${tex_dir}/bibtex/bib//
#export BSTINPUTS=.:/home/jh/lib/texmf/bibtex/bst//:${tex_dir}/bibtex/bst//
#export DVIPSFONTS=${TEXFONTS}:/var/lib/texmf//

# latexcl
rm -f *.bbl \
      *.blg \
      *.dvi \
      *.log \
      *.aux \
      *.ps  \
      *.out \
      *.toc \
      *.lot \
      *.lof

# latex-bibtex-latex-latex-latex:
latex ${root}
bibtex ${root}
for auxfile in chap*.aux
do
    echo $auxfile 
    bibtex `basename $auxfile .aux`
done
latex ${root}
./oedit.py ${root}.out
latex ${root}
latex ${root}

# Generate the pdf file:
dvipdfm ${root}
#latpdf ${root}
#pdflatex ${root}

# Manually rotate necessary pages with Applications -> Graphics -> PDF Editor


# latpdf
#dvips -P pdf -f ${root} | \
#  ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 \
#         -dSubsetFonts=true -dEmbedAllFonts=true - - \
#> ${root}.pdf

